Learning compositional structures for semantic graph parsing

AM dependency parsing is a method for neural semantic graph parsing that exploits the principle of compositionality. While AM dependency parsers have been shown to be fast and accurate across several graphbanks, they require explicit annotations of the compositional tree structures for training. In the past, these were obtained using complex graphbank-specific heuristics written by experts. Here we show how they can instead be trained directly on the graphs with a neural latent-variable model, drastically reducing the amount and complexity of manual heuristics. We demonstrate that our model picks up on several linguistic phenomena on its own and achieves comparable accuracy to supervised training, greatly facilitating the use of AM dependency parsing for new sembanks.

==> decomposition.tex <==
\section{Decomposition algorithm}\label{sec:decomp}

% \begin{figure*}
%     \centering
%     \includegraphics[width=\textwidth]{pics/decomp.pdf}
%     \caption{Semantic graph and its first decomposition steps}
%     \label{fig:provisionalAM}
% \end{figure*}

% purpose
In this section we present a simpler yet more complete method for obtaining an AM dep-tree for a given semantic graph $G$ (for \emph{decomposing} the graph), with much reduced reliance on graphbank-specific heuristics. This method does not specify the source names of the AM dep-tree; we will \emph{learn} meaningful source names jointly with training the parser in \myref{sec:auto} and \myref{sec:neural}.

In this section, we instead use graph-specific \emph{placeholder source names} like in Fig.~\ref{fig:placeholder-graphs}. For each argument slot in a constant, let \nn{n} be the node that eventually fills it in $G$. We write \ps{n} for the placeholder source in that slot; e.g.\ in building the AMR in Fig.~\ref{fig:amr-tinyfairyglows} the source \ps{f} in \H{glow} (Fig.~\ref{fig:placeholder-graphs}) is filled by node \nn{f}, labelled \sent{fairy}. These placeholder sources are not suited to generalize across the corpus or carry linguistic meaning, but they still allow us to track source names across requests and constants to create reentrancies.

% The AM dep-tree created in this section is largely, but not fully, determined by the semantic graph alone. We will see throughout this section what choices remain and in \myref{subsec:latent} how we make them.

% % constants with placeholders (as figures)
% \begin{figure}
% \centering
% \begin{subfigure}[b]{0.19\linewidth}
%     \includegraphics[scale=\defAMRScale]{pics/begin_p.pdf}
%     \caption*{\H{begin}}
% \end{subfigure}
% \begin{subfigure}[b]{0.13\linewidth}
%     \includegraphics[scale=\defAMRScale]{pics/glow_p.pdf}
%     \caption*{\H{glow}}
% \end{subfigure}
% \begin{subfigure}[b]{0.12\linewidth}
%     \includegraphics[scale=\defAMRScale]{pics/tiny_p.pdf}
%     \caption*{\H{tiny}}
% \end{subfigure}
% \begin{subfigure}[b]{0.15\linewidth}
%     \includegraphics[scale=\defAMRScale]{pics/seem_p.pdf}
%     \caption*{\H{seem}}
% \end{subfigure}
% \begin{subfigure}[b]{0.15\linewidth}
%     \includegraphics[scale=\defAMRScale]{pics/fairy.pdf}
%     \caption*{\H{fairy}}
% \end{subfigure}
% \caption{Canonical constants}
% \label{fig:placeholder-graphs}
% \end{figure}
% \begin{figure}
%     \centering
%     \begin{subfigure}[b]{0.19\linewidth}
%     \includegraphics[scale=\defAMRScale]{pics/begin_pp.pdf}
%     \caption*{\Hhat{begin}}
% \end{subfigure}
% \begin{subfigure}[b]{0.135\linewidth}
%     \includegraphics[scale=\defAMRScale]{pics/seem_pp.pdf}
%     \caption*{\Hhat{seem}}
% \end{subfigure}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}


% constants with placeholders (as minipages)
\begin{figure}[t]
\begin{minipage}{0.52\linewidth}
\begin{minipage}[b]{0.26\linewidth}
    \includegraphics[scale=\defAMRScale]{pics/begin_p.pdf}
    \caption*{\small \H{begin}}
\end{minipage}
\begin{minipage}[b]{0.225\linewidth}
    \includegraphics[scale=\defAMRScale]{pics/glow_p.pdf}
    \caption*{\small \H{glow}}
\end{minipage}
\begin{minipage}[b]{0.22\linewidth}
    \includegraphics[scale=\defAMRScale]{pics/tiny_p.pdf}
    \caption*{\small \H{tiny}}
\end{minipage}
\begin{minipage}[b]{0.22\linewidth}
    \includegraphics[scale=\defAMRScale]{pics/seem_p.pdf}
    \caption*{\small \H{seem}}
\end{minipage}
\caption{Canonical constants (we also use {\small$\H{fairy}=\G{fairy}$} from Fig.~\ref{fig:as-graphs})}
\label{fig:placeholder-graphs}
\end{minipage}~
\begin{minipage}{0.45\linewidth}
    \centering
    \begin{minipage}[b]{0.35\linewidth}
    \includegraphics[scale=\defAMRScale]{pics/begin_pp_s.pdf}
    \caption*{\small \Hhat{begin}{1}}
    \end{minipage}
    \begin{minipage}[b]{0.35\linewidth}
    \includegraphics[scale=\defAMRScale]{pics/begin_pp.pdf}
    \caption*{\small \Hhat{begin}{2}}
    \end{minipage}
    \begin{minipage}[b]{0.2\linewidth}
        \includegraphics[scale=\defAMRScale]{pics/seem_pp.pdf}
        \caption*{\small \Hhat{seem}{1}}
    \end{minipage}
    \caption{Non-canonical constants with placeholder sources}
    % \caption{Constants with placeholder sources}
    \label{fig:hbars}
\end{minipage}
\end{figure}



\begin{figure}[t]
% \begin{minipage}{0.38\linewidth}
\begin{subfigure}[t]{0.25\linewidth}
\centering
    \includegraphics[scale=\bigAMRScale]{pics/tinyfairyglowsLine.pdf}  % exists also triangluar shaped tinyfairyglows.pdf
    \caption{AMR}
    \label{fig:amr-tinyfairyglows}
\end{subfigure}
\begin{subfigure}[t]{0.33\linewidth}
\centering
    \includegraphics[scale=\bigAMRScale]{pics/tinyfairyglowsFlipped.pdf}  % exists also triangluar shaped tinyfairyglows.pdf
    \caption{Edge-normalised AMR}
    \label{fig:normalised-tinyfairyglows}
\end{subfigure}
\begin{subfigure}[t]{0.35\linewidth}
\centering
    \begin{forest}
    for tree={align=center, edge=->, font=\small, l sep=1.7em, l=1.7em, }
    [\depNodeWType{\H{glow}}{\type{\ps{f}}}
        [\depNodeWType{\H{fairy}}{\emptytype{}}, name=fairy, edge label = {node [midway, left] {\app{\ps{f}}}}
            [\depNodeWType{\H{tiny}}{\type{\ps{f}}}, edge label = {node [midway, left] {\modify{\ps{f}}}}
            ]
        ]
    ]
    \end{forest}
    \caption{Canonical AM dep-tree with types}
    \label{fig:tree-tinyfairyglows}
\end{subfigure}
\caption{\sent{The tiny fairy glows}.
%Semantic graph without reentrancies and its canonical AM dep-tree.
}
    \label{fig:noReent}
% \end{minipage}~~~~
\end{figure}



\subsection{Basic transformation to AM dep-trees}
Let us first consider the case where the semantic graph $G$ has no reentrancies, like in Fig.~\ref{fig:noReent}a. The first step in obtaining the AM dep-tree for $G$ is to obtain the basic shape of the constants.
We assume that each graph constant contains exactly one labeled node. Each edge belongs to the constant of exactly one node. The edges in the constant of a node are called its \emph{blob} \citep{groschwitz-etal-2017-constrained}; the blobs partition the edge set of the graph. To facilitate presentation, we take the convention in this paper to normalise edges so that they point from the node to whose blob they belong outward, like in Fig.~\ref{fig:noReent}b, where the \el{mod} edge is reversed and grouped with the node \nn{t} to match \H{tiny} in Fig.~\ref{fig:placeholder-graphs}. We add an \textit{-of} suffix to the label of reversed edges (\`a la AMR). Heuristics for this partition of edges into blobs are simple yet effective and therefore a good place to inject linguistic knowledge into the system. Thus, this is the only part of this method where we still rely on graphbank-specific heuristics. (We use the same blob heuristics as \newcite{lindemann-etal-2019-compositional} in our experiments).

% For each edge from a node $n$ to a node $m$ we then have to decide whether the edge goes into the constant of $n$ or $m$. In other words, we decide whether $n$ fills a slot of $m$ or vice versa\todo{use the word blobs}.
Once the decision of which edge goes in which blob is made,
% \todo{should we say here that this is determined heuristically for the whole sembank?}
we obtain what we call \emph{canonical constants}, which are single node constants using placeholder source names and trivial types (i.e.~the empty request at every source); see e.g.~\H{glow} in Fig.~\ref{fig:placeholder-graphs} ($C$ for `canonical'). When we restrict ourselves to the canonical constants, in a setting without reentrancies, the compositional structure is fully determined by the structure of the graph:

\begin{lemma}\label{lem:treeAM}
For a graph $G$ without reentrancies, given a partition of $G$ into blobs, there is exactly one AM dep-tree $t$ with canonical constants that evaluates to it.
\end{lemma}

We call this AM dep-tree $t$ the \emph{canonical AM dep-tree} of $G$. It is isomorphic to $G$, with each node \nn{n} replaced with its canonical constant. Each edge with target \nn{t} is replaced with an \app{\ps{\nn{t}}} edge if it is pointing away from the root of $G$, and with a \modify{\ps{\nn{t}}} edge if it is pointing towards the root. Fig.~\ref{fig:noReent}c shows the sole AM dep-tree evaluating to the graph in Fig.~\ref{fig:noReent}b using the canonical constants in Fig.~\ref{fig:placeholder-graphs}.


% the fairy begins to seem to glow
\begin{figure*}
    \centering
    \begin{subfigure}[t]{0.11\linewidth}
    \centering
    \includegraphics[scale=\defAMRScale]{pics/fairybeginstoseem.pdf}
    \caption{AMR}
    \label{fig:amr-begin-seem}
    \end{subfigure}
    \begin{subfigure}[t]{0.12\linewidth}
    \centering
    \includegraphics[scale=\defAMRScale]{pics/fairybeginstoseemUnrolled.pdf}
    \caption{Unrolled}
    \label{fig:unrolled}
    \end{subfigure}
    \begin{subfigure}[t]{0.23\linewidth}
    \centering
    \begin{forest}
    for tree={align=center, edge=->, font=\small, l sep=1.2em, l=1.2em, }
    [\depNodeWType{\H{begin}}{\type{\ps{s,f}}}, name=begin
        [\depNodeWType{\H{fairy}}{\emptytype{}}, name=fairy, edge label = {node [midway, left] {\small \app{\ps{f}}} }
        ]
        [\depNodeWType{\H{seem}}{\type{\ps{g}}}, edge label = {node [midway, right] {\small \app{\ps{s}}}}
            [\depNodeWType{\H{glow}}{\type{\ps{f}}}, name=glow, edge label = {node [midway, left] {\small \app{\ps{g}}} }
                [\depNodeWType{\refnode{\nn{f}}}{\emptytype{}}, edge label = {node [midway, left] {\small \app{\ps{f}}}}
                ]
            ]
        ]
    ]
    \end{forest}
    \caption{Canonical AM tree for (b)}
    \label{fig:canonical}
    \end{subfigure}
    \begin{subfigure}[t]{0.25\linewidth}
    \centering
    \begin{forest}
    for tree={align=center, edge=->, font=\small, l sep=1.8em, l=1.8em, s sep=0.2em }
    [\depNodeWType{\H{begin}}{\type{\ps{s,f}}}, name=begin
        [\depNodeWType{\H{fairy}}{\emptytype{}}, name=fairy, edge label = {node [midway, left] {\app{\ps{f}}} }
        ]
        [\depNodeWType{\Hhat{seem}{1}}{\type{\ps{g}{\color{blue}\type{\ps{f}}}}}, edge label = {node [midway, right] {\app{\ps{s}}}}
            [\color{blue}\depNodeWType{\refnode{\nn{f}}}{\emptytype{}}, edge = blue, edge label = {node [midway, left] {\color{blue}\app{\ps{f}}}}
            ]
            [\depNodeWType{\H{glow}}{\type{\ps{f}}}, name=glow, edge label = {node [midway, right] {\app{\ps{g}}} }
            ]
        ]
    ]
    \end{forest}
    \caption{$1^{\text{st}}$ percolation step}
    \label{fig:percolated}
    \end{subfigure}
        \begin{subfigure}[t]{0.21\linewidth}
    \centering
    \begin{forest}
    for tree={align=center, edge=->, font=\small, l sep=1.8em, l=1.8em, s sep=0.0em}
    [\depNodeWType{\Hhat{begin}{1}}{\type{\ps{s{\color{blue}\type{\ps{f}}}}, \ps{f}}}, name=begin
        [\depNodeWType{\H{fairy}}{\emptytype{}}, name=fairy, edge label = {node [midway, left] {\app{\ps{f}}} }
        ]
        [\depNodeWType{\Hhat{seem}{1}}{\type{\ps{g\type{\ps{f}}}}}, edge label = {node [midway, right] {\app{\ps{s}}}}
            [\depNodeWType{\H{glow}}{\type{\ps{f}}}, name=glow, edge label = {node [midway, left] {\app{\ps{g}}} }
            ]
        ]
    ]
    \end{forest}
    % \caption{AM dep-tree with place-holder sources}
    \caption{AM dep-tree ($2^{\text{nd}}$ perc)}
    \label{fig:am-placeholder-reent}
    \end{subfigure}
    \caption{\sent{The fairy seems to begin to glow}: AMR and analysis (percolation changes in blue).}
    \vspace{-5pt}
    \label{fig:percolation}
\end{figure*}



\subsection{Reentrancies and types}

Finding AM dep-trees for graphs \emph{with} reentrancies is more challenging. Consider the semantic graph in Fig.~\ref{fig:amr-begin-seem}. The AM dep-tree in Fig.~\ref{fig:am-placeholder-reent} evaluates to it, using some canonical constants but also \Hhat{begin}{1} and \Hhat{seem}{1} from Fig.~\ref{fig:hbars}, which use placeholder sources and complex type requests. In this AM dep-tree, the \ps{f} source of \H{glow} is not filled immediately, but remains unfilled for a while: first, \Hhat{seem}{1} specifies with the request \type{\ps{f}} at its \ps{g} source  that the source should still be unfilled when \Hhat{seem}{1} and \H{glow} combine. The result must keep its source still open when it combines with \Hhat{begin}{1}, due to the $\type{\ps{f}}$ request of \Hhat{begin}{1}. At this point the reentrancy is created and the source  eventually gets filled with \H{fairy}. To obtain this AM dependency tree, one must know which source to add to which requests in which graphs. In some graphs, for example with interacting reentrancies, this can be quite difficult, which is why the heuristics of \newcite{lindemann-etal-2019-compositional} are so complex.
% that it should still be open. while \app{\ps{g}} combines \H{glow} with \Hhat{seem}. 
% It merges eventually with the \ps{f} source of \Hhat{begin} (), creating the reentrancy. This open \ps{f} source is explicitly present in the requests of \Hhat{seem} and \Hhat{begin}.

To solve the problem in its generality, we first \emph{unroll} the graph as in Fig.~\ref{fig:unrolled}, representing the reentrancy not directly, but with a reference node with label \refnode{\nn{f}}. (Merging this node with the node \nn{f} it refers to yields the original graph again.) To get the AM dep-tree in \ref{fig:am-placeholder-reent}, we start with the canonical AM dep-tree of the unrolled graph (Fig.~\ref{fig:canonical}) and then \emph{percolate} the reference node upwards, until the reentrancy is resolved. Each percolation step brings us one step closer to resolving the reentrancy, while leaving appropriate type requests in its trace. This breaks the problem down into simple steps.

In the first percolation step (Fig.~\ref{fig:percolated}), we move the reference constant \refnode{\nn{f}} upwards, attaching it at the constant for \sent{seem} instead of at \H{glow}. This corresponds to delaying filling the \ps{f} source of \H{glow} until after \H{glow} is combined with \H{seem}; we therefore add the $\type{\ps{f}}$ request at the \ps{g} source of \H{seem}, turning it into \Hhat{seem}{1}. This is the general principle of a percolation: moving a reference node upwards in the tree, and adding the appropriate request at its new parent. Note that this does not change the graph denoted by the tree.

In the second percolation step, we similarly add \ps{\nn{f}} to the request of the \sent{seem} source \ps{\nn{s}} in $\H{begin}$, obtaining \Hhat{begin}{1}. But since \H{begin} already has an \ps{f} source, we do not need to move the reference constant \refnode{\nn{f}} up; adding the request already resolves the reentrancy. We therefore simply remove the reference constant and obtain the desired AM dep-tree in Fig.~\ref{fig:am-placeholder-reent}.

Not all percolations are possible. For example, a modifer (i.e.~a node with an incoming \modify{} edge) cannot be percolated up; that would change the evaluation result by changing which node gets modified. We give a technical description of all valid percolations in Appendix~B. 

% \begin{figure}
%     \centering
%     %\includegraphics[width=\textwidth]{pics/decomp.pdf}
%     \caption{Schematic representations of the percolations P1-3. Nodes in the AM dep-trees do not show the constant, but a pair [\nn{n},$tau$] of the graph node corresponding to the constant, and the constant's type (in practice the type may contain additional sources).}
%     \label{fig:percolations}
% \end{figure}

% Fig.~\ref{fig:percolations} shows the three types of percolations \textbf{P1-3} we use to resolve reentrancies. \textbf{P1} and \textbf{P2} are the two steps we saw in the example; \textbf{P3} is like \textbf{P2} but percolates past a \modify{} edge. Due to how \modify{} operations create reentrancies (c.f. Fig.~\todo{background}), no type changes occur in \textbf{P3}. Further, \modify{} cannot change the type of the parent and therefore there is no equivalent to \textbf{P3} where $\nn{g}$ does not have \ps{n} already in its type. Finally, a node with an incoming \modify{} edge can never be percolated up this way (it would change which head the node modifes; i.e.~change the evaluation result).

% \textbf{P1} can percolate up both regular and reference nodes.
We percolate each node and its reference nodes up to their lowest common ancestor, at which point all reentrancies are resolved. If this is not possible with the set of valid percolations, no AM dep-tree can be obtained from this unrolled graph. Non-reference nodes can optionally be percolated beyond the lowest common ancestor. However, we find that linguistic motivation to do so is rare, and always stop percolation at the lowest common ancestor. We leave learning when to perform such optional percolations to future work.
% In Appendix~\todo{}, we introduce one more rare type of percolation \textbf{P4} (\textbf{P4} is not applicable in resolving reentrancies, but can be optionally applied afterwards).

% the fairy that began to glow unrolling and dep trees
\begin{figure}[t]
% \begin{minipage}{0.48\linewidth}
    % \begin{subfigure}[b]{0.34\linewidth}
    % \centering
    % \includegraphics[scale=\defAMRScale]{pics/fairythatbegins.pdf}
    % \caption{AMR}
    % \label{fig:amr-relative}
    % \end{subfigure}
    \hspace{-0.03\linewidth}
    \begin{subfigure}[b]{0.13\linewidth}
    \centering
    \includegraphics[scale=0.41]{pics/fairythatbeginsUnroll1.pdf}
    \caption{}
    \label{fig:amr-relative-unroll1}
    \end{subfigure}
    \begin{subfigure}[b]{0.13\linewidth}
    \centering
    \includegraphics[scale=0.41]{pics/fairythatbeginsUnroll2.pdf}
    \caption{}
    \label{fig:amr-relative-unroll2}
    \end{subfigure}
    \begin{subfigure}[b]{0.245\linewidth}
    \hspace{-50pt}
    \begin{minipage}{\linewidth}
    \begin{forest}
    for tree={align=center, edge=->, font=\small, l sep=1.8em, l=1.8em, }
    [\quad\quad\depNodeWType{\H{fairy}}{\emptytype{}}
        [\quad\quad\depNodeWType{{}\Hhat{begin}{2}}{\type{\ps{f, g\type{\ps{f}}}}}, edge label = {node [midway, right] {\small\modify{\ps{f}}}}
            [\quad\quad\depNodeWType{\H{glow}}{\type{\ps{f}}}, edge label = {node [midway, right] {\small\app{\ps{g}}}}
            ]
        ]
    ]
    \end{forest}
    \end{minipage}
    \centering
    \caption{}
    \label{fig:amr-relative-tree1}
    \end{subfigure}
    \begin{subfigure}[b]{0.265\linewidth}
    \hspace{-40pt}
    \begin{minipage}{\linewidth}
    \begin{forest}
    for tree={align=center, edge=->, font=\small, l sep=1.8em, l=1.8em}
    [\quad\quad\depNodeWType{\H{fairy}}{\emptytype{}}
        [\quad\quad\depNodeWType{\H{glow}}{\type{\ps{f}}}, edge label = {node [midway, right] {\small\modify{\ps{f}}}}
            [\quad\quad\depNodeWType{\H{begin'}}{\type{\ps{g},\ps{f}}}, edge label = {node [midway, right] {\small\modify{\ps{g}}}}]
        ]
    ]
    \end{forest}
    \end{minipage}
    \centering
    \caption{}
    \label{fig:amr-relative-tree2}
   
    \end{subfigure}
    \begin{subfigure}[b]{0.21\linewidth}
    \centering
    \includegraphics[scale=\defAMRScale]{pics/begin_p_fg.pdf}
    % \vspace{1em}
    \caption{\H{begin'}}
    \end{subfigure}

    \caption{Two unrolled graphs (a,b) for \sent{the fairy that begins to glow} (AMR in Fig.~\ref{fig:amr-fairy} above) and (c,d) the resulting AM trees with placeholder source names.}\label{fig:modUnroll}
% \end{minipage}
\end{figure}

\paragraph{Unrolling the graph.} 
Since there are many ways to unroll a graph $G$, it may seem like a wide variety of AM dep-trees could be obtained for $G$ with this procedure, i.e.~that the latent variable space of AM dep-trees with placeholder source names would be large.
However, most choices during unrolling are either unified during upward percolation, or are \emph{invalid} because they do not allow for resolving all reentrancies with valid percolations.

The only meaningful choice comes from complex modifier components as in Fig~\ref{fig:amr-fairy}, where \sent{fairy} is modified by the relative clause \sent{that began to glow} which has two edges to \sent{fairy}. Fig.~\ref{fig:modUnroll} shows how choosing which edge to keep and which we unroll (a,b) yields different AM dependency trees after percolation (c,d; here the former makes more linguistic sense since \sent{began} is the head of \sent{began to glow}). We find that this situation is rare and simply make an arbitrary choice when we encounter it.

For a given graph, we obtain an arbitrary valid unrolled graph by, loosely speaking, traversing the original graph in an arbitrary breadth first order, but prioritizing traversing edges in a forward direction (see Appendix~B for details).

\paragraph{Summary.} In total we use this algorithm $\mathbb{A}$: (1) divide edges into blobs; (2) unroll the graph; and (3) percolate nodes and their referents upwards, resolving reentrancies. $\mathbb{A}$ is correct and complete:

\begin{theorem}\label{thm:correctComplete}
For every graph $G$, every AM dep-tree obtained by algorithm $\mathbb{A}$ is well-typed and evaluates to $G$. By varying the choices for blob partitions, unrolling of complex modifier components, and percolations beyond the lowest common ancestor, every AM dep-tree with single-node constants and placeholder source names can be obtained with algorithm $\mathbb{A}$.
\end{theorem}

% In practice, we use the heuristics of \cite{lindemann-etal-2019-compositional} to divide the edges into blobs. The heuristics define for each edge label whether the edge should be in the blob of its origin or its target. These heuristics are based on the insight that in the AM algebra, edges between a head and a modifier should go with the modifier and edges between a head and an argument should go with the head. This is the only graph-bank specific heuristic of \cite{lindemann-etal-2019-compositional} remaining in the method presented here. 
% % \todo{not quite true. Still have pre- and post-processing of conjunction in SPD, AMR alignments/multi-node constants, and AMR cutting long distance coref. Or are these not heuristics in this sense?}
% Due to the simplicity and effectiveness of these heuristics, we believe this to be an excellent spot to inject linguistic knowledge into the model.

% We find that linguistic motivation for percolations beyond resolving reentrancies is rare, as are complex modifier components as in Fig.~\ref{fig:modUnroll}. We therefore simply never perform the former and make arbitrary choices in the latter situation. Learning to make informed decisions in these rare circumstances could be interesting future work.

% Algorithm $\mathbb{A}$ provides us with an AM tree of fixed structure, but with placeholder source names. Learning meaningful source names that generalize well across the corpus is the topic of the next section.





==> decomposition_old.tex <==
\section{Decomposition algorithm}\label{sec:decomp}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{pics/decomp.pdf}
    \caption{Semantic graph and its first decomposition steps}
    \label{fig:provisionalAM}
\end{figure*}

% purpose
In this section we present a novel algorithm for obtaining all AM dependency trees for a given graph, i.e.~for \emph{decomposing} the graph\todo{we more get any tree than all trees, since we treat only some latent variables as latent; see below}. This algorithm makes explicit the choices during decomposition --i.e.~the latent variables -- in a way that we find to be more useful for unsupervised learning than the method of \cite{groschwitz-etal-2017-constrained}.

% steps
% The algorithm has four steps. First, we fix the constants of the AM dependency tree, using placeholder source names. Then, we draw the edges of the AM tree. Third, we adjust the types of the constants, in particular to account for reentrancies. Finally, we replace the graph-specific placeholder source names with the \sortof{real} source names from a set $\realS$ we use across the corpus. We can show that the following theorem holds:

We first describe the process itself, and then spell out the latent choices in the process and how we adress them. Let us decompose a graph $G$; our running example is shown in Fig.~\ref{fig:provisionalAM}a.
To obtain an AM tree, we first fix its \emph{structure} and the \emph{structure} of its types (in this section). Then we determine what source names, i.e.~the names for the argument and modification slots (Section~\ref{sec:auto}). 

% We can show that the following theorem holds:

% \begin{theorem}\label{thm:correct}
% The algorithm presented here generates exactly all well-typed AM dependency trees (with star-shaped constants over the set of sources $\realS$) that evaluate to $G$.
% \end{theorem}

%is to first generate an AM dependency tree that does not yet resolve reentrancies, but rather creates copies of nodes when a reentrancy occurs in the graph.
%In a second step, the reentrancies are resolved with the AM type system and in a third step, the source names are fixed.

% To be able to refer to nodes in the graph explicitly, we give each node a \emph{node name} \nn{n}; for example, in Fig.~\ref{} the \nl{want} node has node name $w$.


\paragraph{Decomposition overview.}
Determining the \emph{structure} of the AM tree and its types means to determine the whole tree, except that we will be using local \emph{placeholder} source names, rather than source names that generalize across the corpus. This includes determining the graph constants (modulo their source names), the \app{} and \modify{} edges that connect them, and the types of the constants that generate the reentrancies of the graph. We here present a method to obtain exactly all such valid AM trees, discuss which decisions lead to different trees, and then describe how we make those decisions in practice.

\paragraph{Edge attachment.}
The first decision to make is to group nodes and edges into graph constants. We assume that each graph constant contains exactly one node (see Section~\todo{} for how we handle multi-node constants in AMR). For each edge from a node $n$ to a node $m$ we then have to decide whether the edge goes into the constant of $n$ or $m$. In other words, we decide whether $n$ fills a slot of $m$ or vice versa.

Once this decision is made, we obtain the constants in Fig.~\ref{fig:provisionalAM}c for our running example. These constants also use \emph{placeholder source names}; we have one placeholder source name $\ps{\nn{n}}$ for each node $\nn{n}$ in the graph. Note that for each constant, we know for each slot the node $\nn{m}$ that will fill it; we use the placeholder source name $\ps{\nn{m}}$ for that slot. For example, in Fig.~\ref{fig:provisionalAM} we know that the node \exnn{sleep} will fill the slot at the end of the \el{ARG1} edge of the constant $\G{want}^P$ of \exnn{want} (P for \sortof{placeholder source name}); this is simply given in the graph. Thus, we use the placeholder source name $\ps{\exnn{sleep}}$ for this slot in $\G{want}^P$.

To facilitate presentation, we take the convention in this paper to represent each edge as pointing from the node to whose constant it belongs outward, like in Fig.~\ref{fig:provisionalAM}b where the \el{mod} edge is grouped with the \exnn{little} node. We follow the convention of AMR to notate edges that were reversed in this procedure with a \textit{-of} suffix in its label.

\paragraph{Node indexed tree.}
The biggest challenge in creating the AM tree structure is getting the types right to create the correct reentrancies. We solve this by first \sortof{splitting} all reentrancies in the graph to obtain a \emph{node-indexed tree} (Fig.~\ref{fig:provisionalAM}d), then straightforwardly obtaining what we call a \emph{proto-AM-tree} for it (Fig.~\ref{fig:provisionalAM}e), and finally manipulating the proto-AM-tree, adding complex types, such that we obtain an AM-tree that evaluates to the original graph, including the reentrancies (Fig.~\ref{fig:provisionalAM}f).

A node-indexed tree like the one in Fig.~\ref{fig:provisionalAM}d does not represent reentrancies directly, but instead uses \emph{reference nodes} that have special labels, like the node labeled \textsf{REF}-\exnn{cat} here. When merging such a reference node with the node it refers to, one obtains a graph again. We say a node-indexed tree $\Gamma$ is \emph{equivalent} to a graph $G$ if resolving all reference nodes in $\Gamma$ this way yields $G$. Here, the node-indexed tree in (d) is equivalent to the graph in (b).

There are multiple ways of creating a node-indexed tree for a given graph, since all (undirected) cycles in the graph could be split at any node. Further below, we will find that some restrictions apply to the node-indexed tree to obtain only valid AM trees in the and, and we will present a method to obtain all node-indexed trees matching the restrictions there.

\paragraph{Proto-AM-trees.}
We define a \emph{proto-AM-tree} to be an AM tree with placeholder source names and only trivial types (i.e.~all sources have the empty request) that evaluates to a node-index tree.
For a given node-indexed tree $\Gamma$, there is only one proto-AM-tree $\Lambda$ and obtaining it is straightforward. The tree structure of $\Lambda$ and $\Gamma$ is isomorphic and we obtain $\Lambda$ from $\Gamma$ in the following way. First, starting at the root of $\Gamma$, we replace each edge with parent $\nn{p}$ and child $\nn{c}$ with an \app{s\of{\nn{c}}} edge if the edge points downward (i.e.~belongs with the parent) and a \modify{s\of{\nn{p}}} edge if the edge points upward (i.e.~belongs with the child).
Then we replace each node $\nn{n}$ in $\Gamma$ with the canonical constant of $\nn{n}$ according to the edge attachments and placeholder source names given above. The proto-AM-tree that evaluates to the node-indexed tree in Fig.~\ref{fig:provisionalAM}d is shown in Fig.~\ref{fig:provisionalAM}e.

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{pics/unsup2020fig3.jpg}
    \caption{Example of edge percolation\todo{update this to the current notation}}
    \label{fig:upwardsPercSeem}
\end{figure*}


\paragraph{Resolving reentrancies.}

Now we turn the proto-AM-tree into a proper AM tree where the reentrancies of the semantic graph are not encoded with reference nodes, but with the type system of the AM algebra.

First we note that the type system allows us to move edges in the AM tree. Consider the two AM trees in Fig.~\ref{fig:upwardsPercSeem}d and Fig.~\ref{fig:upwardsPercSeem}e. They both evaluate to the graph in Fig.~\ref{fig:upwardsPercSeem}a, but in Fig.~\ref{fig:upwardsPercSeem}e, the \app{\ps{\exnn{cat}}} edge to \extnn{cat} attaches at \extnn{seem} rather than \extnn{sleep}. This is possible because the type at \extnn{seem} expects the source \ps{\exnn{cat}} of \extnn{sleep} to still be open when the two combine. In other words, we delayed filling the \ps{\exnn{cat}} slot, effectively moving the \app{\ps{\exnn{cat}}} edge upwards in the AM tree.

We can use the same principle to remove remove the need for reference nodes. Consider again our proto-AM-tree in Fig.~\ref{fig:provisionalAM}e. We now delay filling the \ps{\exnn{cat}} slot of \extnn{sleep}, moving the reference node up to be a child of \extnn{want}. This adds a \ps{\exnn{cat}} source to the request of \ps{\exnn{sleep}} in the constant for want. Now though, when \sent{sleep} and \sent{want} are combined with the \app{\ps{\exnn{sleep}}} operation, the nodes \ps{\exnn{cat}} of both graphs merge and only one slot for the cat remains; the reentrancy has been created through the type system. We can thus remove the reference-node constant from the tree to obtain the AM tree in Fig.~\ref{fig:provisionalAM}f that evalutes to the orignal semantic graph in Fig.~\ref{fig:provisionalAM}a. \todo{probably need more pictures here.} \todo{Say something somewhere that we don't do renames here.}

\todo{I used node names in the AM tree here, in green. Probably should introduce that somehow, and maybe also use them in the figures.} In general, if we have a node \tnn{\alpha} in an AM tree with an \app{\src{X}}-child \tnn{\beta} that has in turn a \app{\src{Y}}-child \tnn{\gamma}, then we can \emph{percolate \tnn{\gamma} upwards} by adding the \src{Y} annotation to \src{X} in \constof{\tnn{\alpha}} and making \tnn{\gamma} an \app{\src{Y}}-child of \tnn{\alpha}. If, like in the example with $\tnn{\alpha}=\extnn{want}$ we just looked at, \tnn{\alpha} has an
\app{\src{Z}}-child \tnn{\delta} where $\src{Z}$ is a placeholder refering to the same argument as $\src{Y}$, i.e.~$\src{Z}=\ps{\nodeof{\tnn{\gamma}}}$, then we delete \tnn{\gamma} instead of moving it up.

If in this scenario the edge between \tnn{\alpha} and \tnn{\beta} is a \modify{\src{X}} edge instead, then we can do the same percolation to move the \app{\src{Y}} edge up, but only for the case where the \src{Y} source is already contained in the type at \tnn{\alpha} (otherwise, the operation would change the type at \tnn{\alpha}, which is not allowed for \modify{} operations).

% We can percolate the same edge upwards an arbitrary amount of times (keepin the restriction on percolating past \modify{} operations in mind). To properly encode reentrancies and get rid of duplicate nodes, we percolate all AM tree nodes that refer to the same graph node \nn{n} up to their lowest common ancestor. There, all percolation paths meet and only one AM tree node referring to \nn{n} remains.

To resolve all reentrancies, we move each node up to its \emph{percolation target}. The percolation target for a node and all of its reference nodes is their lowest common ancestor. There, all percolation paths meet and only one AM tree node referring to \nn{n} remains. An exception is the case where a reference node $\nn{m}$ to a node $\nn{n}$ is a descendent of $\nn{n}$ itself. In that case, we can show that we can assume\todo{assume for what?} that $\nn{m}$ is a descendant of a modifier of \nn{n}, and that it is enough to percolate \nn{m} upwards to that modifier.\todo{example?}\todo{I haven't fully figured out yet what happens in this example, but I don't think it's too complicated}


We can optionally perform percolations beyond the percolation target; this is another latent variable in the AM tree.

\todo{Rare cornercase: can do swap of two \modify{} edges (one becomes \app{}), this corresponds to optional percolation.}

\paragraph{Restrictions.} % restrictions on proto-AM-tree and node indexed tree
The fact that the above percolations are not always possible present restrictions on the proto-AM-tree and thus the node-indexed tree. This is because if a node in a proto-AM-tree $\Lambda$ cannot be percolated to its percolation target, then we cannot obtain a valid AM tree from $\Lambda$. We thus translate the percolation restrictions given above into properties of the proto-AM-tree and the node-indexed tree, and ensure we only obtain trees matching those properties.

First, only \app{} edges can be percolated upwards. In the proto-AM-tree, this means that all nodes that must be percolated upwards, in particular all reference ndoes, must have incoming \app{} edges. In the node-indexed tree, all such nodes must be connected to their parent with an edge that points towards them.

Furthermore, we saw that if an AM-tree node $\tnn{\alpha}$ referring to a node \nn{n} must be percolated \emph{past} a \modify{} edge $e$, the parent \tnn{\beta} (in the AM tree) of $\tnn{\alpha}$ must already have the placeholder source \ps{\nn{n}} in its type. The type of \tnn{\beta} can only have this source if \tnn{\beta} has a tree node referring to \nn{n} as an \app{} child, modifies such a tree node, or \ps{\nn{n}} has been added by a percolation through an \app{} edge.

In the proto-AM-tree we can formulate this as the following property. For every AM-tree node \tnn{\alpha} with percolation target \tnn{\beta}, and for every \modify{} edge $e$ on the path $p$ from \tnn{\beta} to \tnn{\alpha}, one of the following must be true: \tnn{\beta} has a tree node referring to the same node as \tnn{} as an \app{} child, modifies such a tree node, or there must be a tree node \tnn{\gamma} referring to the same node as \tnn{\alpha} and also having percolation target \tnn{\beta}, such that the path $p'$ from \tnn{\beta} to \tnn{\gamma} is identical to $p$ up to (excluding) the \modify{} edge $e$, and $p'$ has only \app{} edges after that.

\todo{Probably don't need this duplication fully spelled out?} In the node-indexed tree, this translates to the following property. For every tree node \nn{a} with percolation target \nn{b}, for every upward edge $e$ on the path $p$ from \nn{b} to \nn{a}, one of the following must be true: \nn{b} has a node referring to \nn{a} as a dependent of a downward pointing edge, is the child of such a node with an upward pointing edge, or there must be another node \nn{c} referring to the same node as \nn{a} and also having percolation target \nn{b}, such that the path $p'$ from \nn{b} to \nn{c} is identical to $p$ up to (excluding) the upwards edge $e$, and $p'$ has only downward edges after that.

\todo{Without loss of generality, we can assume that no reference node has an outgoing edge in the node-index tree, since all tree nodes referring to the same original graph node get unified in the end anyway. And indeed, the algorithm below gives us only such trees. I'm not sure if this is something that needs to be said.}

\paragraph{Obtaining the node indexed tree}
We obtain a node-index tree with the desired properties using the following algorithm (the proto-AM-tree then inherits the properties automatically).

We process all edges of the semantic graph (with edge directions normalized with respect to constant-attachment), starting at the root, adding edges and nodes to the node-indexed tree as we go.

\todo{this, and particularly the paragraph after, may be hard to understand without pictures. I don't know if we can cut it; if we don't I'll add pictures or reuse the given example}
In a first pass, we only travel along edges in forward direction. We add all edges and nodes that we encounter to the node-indexed tree $\Gamma$. When we encounter a node a second time, we add a reference node to $\Gamma$ instead and we don't travel through the outgoing edges a second time. All edges added this way correspond to downward edges in the node-index tree and thus \app{} edges in the proto-AM-tree. Therefore, all nodes and reference nodes added this way can be straightforwardly percolated to their percolation target.

After this procedure is complete, several connected components of not yet processed nodes may remain, that could not be reached by going through edges in forward direction (such as \exnn{little} in Fig.~\ref{fig:provisionalAM}b). Each such component $C$ is connected to the component $M$ of already processed nodes by edges pointing from $C$ to $M$ (if the edge went the other way, it would have been covered in the first, \sortof{forward} pass). We define $D$ to be the set of nodes in $M$ that have an incoming edge from $C$, and define $\nn{x}$ as their lowest common ancestor in $M$. We then pick one edge from $C$ to $\nn{x}$ and split all other edges from $C$ to $M$, introducing reference nodes for the nodes in $M$ where we split\todo{example}. The connecting edge between $C$ and $M$ must connect at $\nn{x}$, because \todo{}. If there is no edge from $C$ to $\nn{x}$, there is no AM tree evaluating to the semantic graph using the edge-constant groupings made above, and the decomposition fails. If there are multiple such edges, each is a valid choice and we obtain structurally different AM trees depending on which one we pick. %In practice, we find that this occurs very rarely and we simply select an arbitrary edge.

We then iterate this process for the component $C$, using the node connected to $\nn{x}$ as the new root; we continue this process until all nodes and edges are covered. We present a technical description of this procedure, and a proof that it yields exactly all node-indexed trees with the desired properties, in Appendix~\todo{}



\paragraph{Theoretical guarantees.}
We show that the above algorithm is correct and complete; that is, every AM tree obtained with the algorithm is well-typed and evaluates to the given graph, and we can obtain every such AM tree with the algorithm. We present a proof sketch here and a full proof in Appendix~\todo{}.

The key for proving correctness is to realize that the upwards percolation of edges does not affect well-typedness, and that the evaluation result stays the same modulo merging of reference nodes. Since the proto-AM-tree is well-typed and evaluates to the node-indexed tree which in turn is equivalent modulo reference nodes to the original graph, and since after all necessary percolations no reference nodes remain, the final AM tree must evaluate to the original graph.

To show that we can find \emph{all} valid AM trees this way, we first take any valid AM tree $t$ as given. We then perform the edge percolation in inverse, obtaining a proto-AM-tree from which we can obtain $t$ and for which we can show that it satisfies the properties we requested above. Since we can obtain any such proto-AM-tree with the above method (c.f.~Appendix~\todo{}), we can also obtain the one leading to $t$, and therefore obtain $t$.

\paragraph{Algorithm summary and latent variables.}
In practice, we first obtain the edge-constant groupings
using the heuristics of \cite{lindemann-etal-2019-compositional} that for each edge label define whether the edge should go with its origin or its target. These heuristics are based on the insight that in the AM algebra, edges between a head and a modifier should go with the modifier and edges between a head and an argument should go with the head. This is the only graph-bank specific heuristic of \cite{lindemann-etal-2019-compositional} remaining in the method presented here. Due to the simplicity and effectiveness of the heuristics, we believe this to be an excellent spot to inject linguistic knowledge into the model.

From there, we obtain graph constants with placeholder source names deterministically as discussed above. We then obtain a single node-indexed tree with the above method. The case where there are multiple valid edge connections for a secondary component is rare, and we simply make an arbitrary choice.

From there, we again deterministically obtain a proto-AM-tree and percolate all nodes to their percolation target. Situations where percolations beyond that make linguistic sense are again rare \todo{say something about it?} and we simply never perform such optional percolations. We leave the development of methods for deciding when to perform optional percolations to future work.

This algorithm provides us with an AM tree of fixed structure, but with placeholder source names. Learning source names that generalize well across the corpus is the topic of the next section.

% \paragraph{Latent variables and solutions.}
% The above algorithm has the following points where choices are made:
% \begin{enumerate}
%     \item The choice to which node each edge attaches in the constants,
%     \item Choosing the root of each component during backward expansion,
%     \item Optional upward percolations, and
%     \item Mapping placeholder source names to generalizable source names.
% \end{enumerate}

% As discussed above, we choose edge-constant attachment with the same heuristics as \cite{lindemann-etal-2019-compositional}. 
% %This is the only graphbank-specific heuristic left. It is a rather straightforward heuristic (attach head-argument edges to the head and head-modifier edges to the modifier; the heuristic consists of defining which edge labels correspond to head-argument edges and which to head-modifier edges) and does not require intimate knowledge of the AM algebra.

% The next two latent variables -- choosing a root in backwards percolation and optional percolation -- are rare. We leave a thorough treatment of them to future work; we simply never percolate and always pick an arbitrary root.

% This leaves the latent choice of mapping placeholder source names to generalizable source names, which is the topic of the next section. 

% \todo{move this somewhere else maybe? Or say something else about it} Since renames are rare (this is visible in the data using the heuristic annotations of \cite{lindemann-etal-2019-compositional}, as well as in \cite{groschwitz-etal-2017-constrained} who use renames only for object-control verbs) and increase the latent variable space by a large margin \todo{how much?}, we make the simplifying assumption to not allow renames at all.


% \paragraph{Constants and \DAG.}
% % constants
% We restrict our decomposition to only use star-shaped constants (this corresponds in particular to predicting at most one labeled graph node per word; we relax this restriction in Section~\ref{subsec:alignmentsAndMultinode} below). We obtain those constants by creating one constant \constof{\nn{n}} for each node \nn{n} in $G$ (using \nn{n} as the labeled node) and deciding for each edge of $G$, to which constant of its incident nodes it belongs. This neatly partitions the graph into constants. 

% Note that each slot in a constant corresponds to a real node in the graph $G$; we know which node will fill it eventually. Our placeholder source names based on this insight. For each slot in a constant \constof{\nn{n}} that gets filled with a node \nn{m}, we create a placeholder source name \plholder{\nn{n}}{\nn{m}} to label that slot. For the example graph in Fig.~\ref{fig:provisionalAM}a, this gives us the constants in Fig.~\ref{fig:provisionalAM}b.

%Furthermore, we create as an auxiliary structure a directed acyclic graph we call \emph{\DAG}. It has the same nodes as $G$ (and the same root), but it has an edge from node \nn{n} to \nn{m} if and only if \nn{m} fills a slot of the constant \constof{\nn{n}} (one can see that this gives the same edges as in $G$, but unlabeled and possibly with a different direction). An example \DAG can be seen in Fig.~\ref{fig:provisionalAM}c (we use \exnn{want} etc.~as names for the nodes in the graph in Fig.~\ref{fig:provisionalAM}a). We write $\args{\nn{n}}$ for the set of nodes (like \nn{m}) that fill the slots in the constant \constof{\nn{n}}.


% \subsection{Creating the preliminary AM dependency tree}

% % Basic idea of provisional AM dep
% The basic idea to create the provisional AM dependency tree is that we start at the root of the \DAG and traverse all its edges exactly once. When we traverse an edge, we add an \app{} edge to the AM tree if we traverse it in forward direction and add a \modify{} edge if we traverse it in backward direction. When we encounter a node \nn{n}, we add a node \tnn{\alpha} to the AM dependency tree that has \nn{n} and its constant assosiated with it; $\nodeof{\tnn{\alpha}}=\nn{n}$ and $\constof{\tnn{\alpha}}=\constof{\nn{n}}$. When we encounter a node \nn{n} a second time, we simply add a new node to the AM dependency tree that refers to \nn{n} and \constof{\nn{n}} again; we take care of these duplicates in Section~\ref{subsec:reent}.

% \begin{algorithm}[t]
% \algrenewcommand\algorithmicindent{1.0em}%
% \newcommand{\seen}[0]{{\small{\textsf{seen}}}}
% \newcommand{\exclude}[0]{{\small{\textsf{excl}}}}
% \newcommand{\seenLocal}[0]{{\small{\textsf{seenLocal}}}}
% \begin{algorithmic}[1] 

% % 		\Function{provisionalTree}{$G$}
% % 		\State $\nn{r}\leftarrow\text{ root of }G$
% % 		\State $T\leftarrow\text{ new empty AM depenency tree}$
% % 		\State add new node $\tnn{\alpha}$ to $T$ with $\nodeof{\tnn{\alpha}}=\nn{r}$
% % 		\State ${\small \textsc{expand}}\of{G,T,\tnn{\alpha}, \emptyset, \emptyset}$
% % 		\State\Return $T$
		
% % 		\EndFunction
		
% % 		\State

% 		\Function{expand}{$G,T,\tnn{\alpha},\seen, \exclude$}
% 		\State $\seenLocal\leftarrow {\small \textsc{expFwd}}\of{G,T,\tnn{\alpha}, \seen, \exclude}$
% 		\State ${\small \textsc{expBwd}}\of{G,T,\tnn{\alpha}, \seen, \seenLocal}$
		
% 		\EndFunction
		
% 		\State
		
% 		\Function{expFwd}{$G,T,\tnn{\alpha},\seen, \exclude$}
% 		\State $\seenLocal \leftarrow \emptyset$
% 		\State $\nn{n}\leftarrow\nodeof{\tnn{\alpha}}$
% 		\For{$\nn{m}\in \args{\nn{n}}\setminus\exclude$}\label{step:iterFwd}
% 		    \State Add new node \tnn{\beta} to $T$ with $\nodeof{\tnn{\beta}}=\nn{m}$\label{step:fwdAddStart}
% 		    \State Add new edge \depedge{\tnn{\alpha}}{\tnn{\beta}}{\app{\plholder{\nn{n}}{\nn{m}}}} to $T$\label{step:fwdAddEnd}
% 		    \If{not $\nn{m}\in\seen$}\label{step:fwdRecursionStart}
%     		    \State add \nn{m} to \seen~and \seenLocal
%     		    \State ${\small{\textsf{new}}} \leftarrow {\small\textsc{expFwd}}\of{G,T,\tnn{\beta}, \seen, \emptyset}$
%     		    \State $\seenLocal\leftarrow\seenLocal\cup {\small{\textsf{new}}}$
%     		\EndIf\label{step:fwdRecursionEnd}
% 		\EndFor
% 		\State \Return \seenLocal
% 		\EndFunction
		
% 		\State 
		
% 		\Function{expBwd}{$G,T,\seen, \seenLocal$}
% 		\For{connected component $C$ in $G\setminus\seen$ such that $C$ is adjacent to \seenLocal}
%     		\State $\tnn{\alpha}\leftarrow{\small\textsc{findParent}\of{T,\seenLocal,C}}$
%     		\State $\nn{x}\leftarrow \nodeof{\tnn{\alpha}}$
%     		\State $\nn{r}\leftarrow{\small\textsc{pickRoot}\of{x,C}}$
%     		\State Add new node \tnn{\beta} to $T$ with $\nodeof{\tnn{\beta}}=\nn{r}$
% 		    \State Add new edge \depedge{\tnn{\alpha}}{\tnn{\beta}}{\modify{\plholder{\nn{x}}{\nn{r}}}} to $T$
% 		    \State add \nn{r} to \seen
%     		\State ${\small\textsc{expand}}\of{G,T,\tnn{\beta},\seen,\{\nn{x}\}}$
% 		\EndFor
% 		\EndFunction
% 	\end{algorithmic}
% \caption{Obtaining the provisional AM dependency tree.}\label{alg:provisionalAMdep}
% \end{algorithm}

% % Details of provisional AM dep
% Algorithm~\ref{alg:provisionalAMdep} details this procedure. To obtain the provisional AM dependency tree for a graph $G$, we start with an AM dependency tree $T$ that contains only a node \tnn{\alpha} corresponding to the root of $G$ and call $\textsc{expand}\of{G,T,\tnn{\alpha},\emptyset,\emptyset}$. This expands the tree $T$ recursively. To make sure we only obtain valid AM trees (i.e.~that Theorem~\ref{thm:correct} holds), we must take care in which order we traverse the edges. The principle of Algorithm~\ref{alg:provisionalAMdep} is that our expansion has two steps. First, \textsc{expandFwd} traverses all edges that can be traversed in a forward direction from the root. Then \textsc{expandBwd} allows just one backward traversal into each remaining connected component. Then for each such connected component, the whole expansion process starts over -- first as far as possible forward, then up to one step backward into each remaining component -- with a newly picked local root in the component. The sets \textsf{seen}, \textsf{seenLocal} and \textsf{excl} make sure we don't add spurious duplicate edges and nodes to the AM tree $T$.

% \paragraph{Example.} Let us walk through an example where $G$ is the graph in Fig.~\ref{fig:provisionalAM}a. The root of $G$ is \exnn{want} and we start with a tree node \extnn{want} corresponding to it. We then \textsc{expand} \extnn{want}. The recursive (c.f.~Line~\ref{step:fwdRecursionStart}) forward expansion encounters \exnn{sleep} once and \exnn{cat} twice (once as an argument of \exnn{want} and once as an argument of \exnn{sleep}), creating the nodes \extnn{sleep}, \extnn{cat1} and \extnn{cat2} as well as the corresponding \app{} edges (result in \todo{Fig.~\ref{}; imagine Fig.~\ref{fig:provisionalAM}d without \extnn{tired} for now}; c.f.~Lines~\ref{step:fwdAddStart}-\ref{step:fwdAddEnd}).



% Now, the node \exnn{tired} is not taken care of yet, since we can reach it from the root only by going \emph{backwards} through a DAG edge. This is what the \textsc{expBwd} function does. Once the forward expansion stops, it looks at all connected components $C$ of nodes that are not covered yet; each backward expansion only considers components adjacent to nodes seen in the forward expansion that preceded it (tracked by the \textsf{seenLocal} set). Here, there  is exactly one such component containing exactly the \nl{tired} node. For this component, we first find the node where the component attaches in $T$, here this is \extnn{cat1}, and then choose a local root of the component, here \exnn{tired}. We connect the two with a \modify{\plholder{\exnn{tired}}{\exnn{cat}}} edge. As in the forward expansion, we label the corresponding slot in the corresponding constant accordingly.
% The recursive call of \textsc{expand} for the component would normally add another copy of \exnn{cat} as a child of \extnn{tired} in the forward pass; to avoid this spurious edge, we explicitly exclude the parent \nn{x} as a child of the local root \nn{r} in the forward expansion. This concludes the full expansion process, with the result shown in Fig.~\ref{fig:provisionalAM}d.

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{pics/unsup2020fig2.jpg}
%     \caption{\DAG{s} with complex backward expansion}
%     \label{fig:backwardExp}
% \end{figure}

% \paragraph{Details of backward expansion} The backward expansion is not always so straightforward as in this example and we use a general procedure to handle complex situations like the ones in Fig.~\ref{fig:backwardExp} (we only print the \DAG{s} for simplicity). The general rule for \textsc{findParent} is deterministic: first, we define a set $D$ of all nodes added during the last forward pass (i.e.~the nodes in $T$ corresponding to graph nodes in \textsf{seenLocal}) that have a direct edge from the component $C$. We call the nodes in $D$ \emph{docking points}. If multiple such AM tree nodes correspond to the same graph node, only the first one we added to the AM tree $T$ is a docking point and in $D$. Then the parent is the lowest common ancestor (in the \DAG) of the docking points. Take for example the graph in Fig.~\ref{fig:backwardExp}a, here $\nn{a}$ is the root of the graph and the forward pass covers $\nn{a}$ and $\nn{b}$. The backward pass then has the component $\{\nn{c},\nn{d}\}$ and both $\nn{a}$ and $\nn{b}$ are connected to them with edges; therefore the docking pints are $D=\{\nn{a},\nn{b}\}$ and the parent, as their lowest common ancestor, is $\nn{a}$. In Fig.~\ref{fig:backwardExp}b, the forward pass covers $\nn{a}$, $\nn{b}$ and $\nn{c}$ and we add $\nn{d}$ in the backward pass; here then $D=\{\nn{b},\nn{c}\}$ and the parent is $\nn{a}$.

% In contrast to the choice of the parent, the choice of the component-root is not always deterministic; at first glance it could be any node in the component. However, note that since the component-root attaches to the parent with a \modify{} operation, it must have a slot for the parent. But if it has no edge to it in the \DAG that is not the case and we cannot find a well-typed AM dependency tree for this scenario. Thus, we can choose as component-root exactly the nodes in the component that have an edge to the parent in the \DAG. For example, in Fig.~\ref{fig:backwardExp}a, only $\nn{c}$ can be the component-root. By contrast in Fig.~\ref{fig:backwardExp}c, the component is $\{\nn{b},\nn{c}\}$ and both nodes have an edge to the parent $a$, i.e.~both are valid choices for the component-root. If we choose $\nn{c}$ as the component root, $\nn{b}$ is added as its \app{}-child in the subsequent forward expansion; if we choose $\nn{b}$ as the component root, then $\nn{c}$ is added as its modifier in the subsequent backward expansion. We thus obtain different AM dependency trees for different choices of component roots. 

% This is also a point when the decomposition can fail, for example in Fig.~\ref{fig:backwardExp}b the only node in the component is $\nn{d}$ but it is not a valid choice as component-root. In particular, the lowest common ancestor of the docking points must itself be a docking point, or else the decomposition fails.



% \subsection{Resolving reentrancies}\label{subsec:reent}

% \begin{figure*}
%     \centering
%     \includegraphics[width=\textwidth]{pics/unsup2020fig3.jpg}
%     \caption{Example of edge percolation}
%     \label{fig:upwardsPercSeem}
% \end{figure*}

% \begin{figure*}
%     \centering
%     \includegraphics[width=\textwidth]{pics/unsup2020fig4.jpg}
%     \caption{Resolving reentrancies}
%     \label{fig:upwardsPercWant}
% \end{figure*}

% The AM dependency tree that we built so far (Fig.~\ref{fig:provisionalAM}d) still contains duplicate nodes where there should be reentrancies; if we were to evaluate it we would get the incorrect result in Fig.~\ref{fig:provisionalAM}e. However, the type system of the AM algebra allows us to resolve these reentrancies; we develop the method for that in this section.

% First we note that the type system allows us to move edges in the AM tree. Consider the two AM trees in Fig.~\ref{fig:upwardsPercSeem}d and Fig.~\ref{fig:upwardsPercSeem}e. They both evaluate to the graph in Fig.~\ref{fig:upwardsPercSeem}a, but in Fig.~\ref{fig:upwardsPercSeem}e, the \app{\plholder{\exnn{sleep}}{\exnn{cat}}} edge to \extnn{cat} attaches at \extnn{seem} rather than \extnn{sleep}. This is possible because the type at \extnn{seem} expects the source \plholder{\exnn{sleep}}{\exnn{cat}} of \extnn{sleep} to still be open when the two combine. In other words, we delayed filling the \plholder{\exnn{sleep}}{\exnn{cat}} slot, effectively moving the edge upwards in the AM tree.

% We can use the same principle to remove duplicate nodes to resolve reentrancies. Consider again our provisional AM tree in Fig.~\ref{fig:provisionalAM}d. We now want to delay filling the \plholder{\exnn{sleep}}{\exnn{cat}} slot of \extnn{sleep}. We use a slight variant of the above method for this, with the result shown in Fig.~\ref{fig:upwardsPercWant}(a,b). The principle of adding an annotation to here \extnn{want} that requires the \plholder{\exnn{sleep}}{\exnn{cat}} slot of \extnn{sleep} to remain open is the same. But there are two major differences. First, we add a rename annotation $[\plholder{\exnn{sleep}}{\exnn{cat}}\renamearrow\plholder{\exnn{want}}{\exnn{cat}}]$ to \extnn{want} (see the constant in Fig.~\ref{fig:upwardsPercWant}b) that ensures that the two slots of \constof{\extnn{want}} and \constof{\extnn{sleep}} that will be filled with \exnn{cat} merge. Second, we do not move the node \extnn{cat2} up, but rather delete it; since the \plholder{\exnn{sleep}}{\exnn{cat}} slot of \constof{\extnn{sleep}} merged with the respective slot of \constof{\extnn{want}}, it will automatically be filled when \extnn{want} and \extnn{cat1} combine. In a situation where \extnn{cat2} would have outgoing edges, we would attach those edges to \extnn{cat1} instead so they do not get lost.

% Another option here is to make the simplifying assumption that no renames occur and that the involved source names must instead be the same. In this example, this means we assume $\plholder{\exnn{want}}{\exnn{cat}}=\plholder{\exnn{sleep}}{\exnn{cat}}$. We obtain the same AM tree in Fig.~\ref{fig:upwardsPercWant}a again, but now with the constants in Fig.~\ref{fig:upwardsPercWant}c. (Without this assumption we can still arrive at the same result eventually if both placeholder source names get mapped to the same \sortof{real} source name later.)

% In general, if we have a node \tnn{\alpha} with an \app{\src{X}}-child \tnn{\beta} that has in turn a \app{\src{Y}}-child \tnn{\gamma}, then we can \emph{percolate \tnn{\gamma} upwards} by adding the \src{Y} annotation to \src{X} in \constof{\tnn{\alpha}} and making \tnn{\gamma} an \app{\src{Y}}-child of \tnn{\alpha}. If, like in the example with $\tnn{\alpha}=\extnn{want}$ we just looked at, \tnn{\alpha} has an
% \app{\src{Z}}-child \tnn{\delta} where $\src{Z}$ is a placeholder refering to the same argument as $\src{Y}$, i.e.~$\src{Z}=\plholder{\nn{n}}{\nodeof{\tnn{\gamma}}}$, then we instead delete \tnn{\gamma}, add its children to \tnn{\delta}, and either add the rename annotation $[\src{Y}\renamearrow\src{Z}]$ to \src{X} in \constof{\tnn{\alpha}} or make the simplifying assumption $\src{Y}=\src{Z}$.

% If in this scenario, the edge between \tnn{\alpha} and \tnn{\beta} is a \modify{\src{X}} edge instead, then we can do the same percolation, but only for the case where such a \app{\src{Z}}-child \tnn{\delta} exists (otherwise, the operation would change the type at \tnn{\alpha}, which is not allowed for \modify{} operations) and since renames are not allowed in \modify{} operations, we in this case \emph{must} make the assumption $\src{Y}=\src{Z}$.

% We can percolate the same edge upwards an arbitrary amount of times (keepin the restriction on percolating past \modify{} operations in mind). To properly encode reentrancies and get rid of duplicate nodes, we percolate all AM tree nodes that refer to the same graph node \nn{n} up to their lowest common ancestor. There, all percolation paths meet and only one AM tree node referring to \nn{n} remains.

% We can optionally perform percolations beyond that point; this is another latent variable in the AM tree.

% We cannot percolate \modify{} edges, but we can show that when a graph node is referenced multiple times in the AM tree, then the incoming edges of all its occurences are \app{} edges.

% \todo{Rare cornercase: can do swap of two \modify{} edges (one becomes \app{}), this corresponds to unforced percolation.}


% \subsection{The latent variables}~\label{subsec:latent}
% The above algorithm has the following points where choices are made:
% \begin{enumerate}
%     \item The choice of edge direction in the \DAG (i.e.~to which node each edge attaches in the constants),
%     \item Choosing the root of each component during backward expansion,
%     \item Optional upward percolations, and
%     \item Mapping placeholder source names to generalizable source names.
% \end{enumerate}

% We choose edge direction in the \DAG with the same heuristics as \cite{lindemann-etal-2019-compositional}. This is the only graphbank-specific heuristic left. It is a rather straightforward heuristic (attach head-argument edges to the head and head-modifier edges to the modifier; the heuristic consists of defining which edge labels correspond to head-argument edges and which to head-modifier edges) and does not require intimate knowledge of the AM algebra.

% The next two latent variables -- choosing a root in backwards percolation and optional percolation -- are rare. We leave a thorough treatment of them to future work; we simply never percolate and always pick an arbitrary root.

% This leaves the latent choice of mapping placeholder source names to generalizable source names, which is the topic of the next section. Since renames are rare (this is visible in the data using the heuristic annotations of \cite{lindemann-etal-2019-compositional}, as well as in \cite{groschwitz-etal-2017-constrained} who use renames only for object-control verbs) and increase the latent variable space by a large margin \todo{how much?}, we make the simplifying assumption to not allow renames at all.


% \subsection{Stuff}

% \todo{a comment on unforced percolation} In the case where alignments are given, we also experiment with a graphbank-independent heuristic, where we perform optional percolation greedily if and only if the percolation reduces the number of non-projective edges in the AM dependency tree (this matches the intuition in the raising case shown above).

% \todo{a comment on unforced percolation and \modify{} root}
% Both of these latent variables might benefit from more complex modelling, but since they are both complex and rare, we leave that to future work.

==> old_stuff.tex <==
%%%%%%%%%%%%%    from decomposition

% , i.e.~for \emph{decomposing} the graph\todo{we more get any tree than all trees, since we treat only some latent variables as latent; see below}. This algorithm makes explicit the choices during decomposition --i.e.~the latent variables -- in a way that we find to be more useful for unsupervised learning than the method of \cite{groschwitz-etal-2017-constrained}.

% We first describe the process itself, and then spell out the latent choices in the process and how we adress them. Let us decompose a graph $G$; our running example is shown in Fig.~\ref{fig:provisionalAM}a.
% To obtain an AM tree, we first fix its \emph{structure} and the \emph{structure} of its types (in this section). Then we determine what source names, i.e.~the names for the argument and modification slots (Section~\ref{sec:auto}). 

% We will at points also use \emph{placeholder source names}; we have one placeholder source name $\ps{\nn{n}}$ for each node $\nn{n}$ in the graph. Note that for each constant, we know for each slot the node $\nn{m}$ that will eventually fill it in the final graph; we use the placeholder source name $\ps{\nn{m}}$ for that slot. For example, in Fig.~\ref{fig:provisionalAM} we know that the node \exnn{sleep} will fill the slot at the end of the \el{ARG1} edge of the constant $\G{want}^P$ of \exnn{want} (P for \sortof{placeholder source name}); this is simply given in the graph. Thus, we use the placeholder source name $\ps{\exnn{sleep}}$ for this slot in $\G{want}^P$.
%We call the constants with placeholder source names and no type annotations the \emph{canonical constants} \todo{maybe later? this relies on a fixed edge-constant grouping / blob partition}. We write $\constof{\nn{n}}$ for the canonical constant of a graph node $\nn{n}$. \todo{say somewhere what the placeholder source names are for, and that we will later replace them with source names that are consistent across the corpus}


% We use the following \textbf{Algorithm 1} to obtain exactly the unrolled graphs that lead to valid AM dep-trees. \todo{somehow visually separate the algorithm description from the rest?}

% \begin{figure}
%     \centering
%     % \includegraphics{}
%     \caption{(a) Graph $G$, (b) after forward expansion and (c) fully unrolled. We leave out node labels here for readability.}
%     \label{fig:unroll}
% \end{figure}

% Consider the graph $G$ in Fig~\ref{fig:unroll}a as an example. We start at the root $a$ of $G$ and perform a \emph{forward expansion}, where we traverse edges in forward direction and breadth first order as far as possible. We add nodes and edges to the unrolled graph $U$ as we pass them. When we see a node for the second time, we add a reference node to $U$ instead (and don't traverse the node's outgoing edges again); see Fig~\ref{fig:unroll}b for the result. The exact order of this expansion does not matter, since a node and all its reference will get percolated up to the same lowest common ancestor in any case.

% This forward expansion may leave us with several connected components $C_i$ of nodes that have not been traversed; here, we have one such component $C_0$ containing exactly the node \nn{d}. Each edge connecting a $C_i$ to the rest of the graph has its origin in $C_i$ (if the edge went the other way, it would have been traversed during the forward expansion). We write $D_i$ for the set of nodes not in $C_i$ with an incoming edge from $C_i$; in this example, $D_0=\left\{\nn{a},\nn{c}\right\}$. We then traverse one edge from the \emph{lowest common ancestor} of $D_i$ into $C_i$ -- this traverses the edge in backwards direction -- arriving at a node $r_i$. We then continue the forward expansion process starting at $r_i$, continuing this iteration until all nodes are covered. In the example, the lowest common ancestor of $D_0$ is \nn{a}, and we accordingly traverse from \nn{a} to $r_0=\nn{d}$, traversing backwards across the edge. We then continue the forward expansion from there, adding a reference node to \nn{c} and obtaining the final unrolled graph in Fig~\ref{fig:unroll}c.

% Note that the backwards traversed edge between \nn{a} and \nn{d} turns into a \modify{} edge in the canonical AM dep-tree, since it points towards the root. Further recall that we can percolate \refnode{\nn{c}} past that edge only if the constant \constof{\nn{a}} its parent \nn{a} has an \ps{\nn{c}} source. This is not the case naturally -- \constof{\nn{a}} has arguments \nn{b} and \nn{e} -- but we can get the source \ps{\nn{c}} in there by percolating \nn{c} upwards past \nn{b}. This is possible because \nn{a} is an ancestor of \nn{b}, which is why we choose the lowest common ancestor of $D_i$ as the node from which to traverse into $C_i$. If there are multiple edges from $C_i$ to that lowest common ancestor, we can choose any one, each yielding a different AM dep-tree in the end. If there is no such edge, there is no AM dep-tree for this choice of blob partition and the decomposition fails.


% Finding AM dep-trees for graphs \emph{with} reentrancies is more challenging. Before we tackle that challenge, we first make the observation that the type system in the AM algebra essentially allows nodes to move upward in the AM dep-tree by delaying their application. Consider the two AM trees in Fig.~\ref{fig:upwardsPercSeem}d and Fig.~\ref{fig:upwardsPercSeem}e. They both evaluate to the graph in Fig.~\ref{fig:upwardsPercSeem}a, but in Fig.~\ref{fig:upwardsPercSeem}e, the \app{\ps{\exnn{cat}}} edge to \extnn{cat} attaches at \extnn{seem} rather than \extnn{sleep}. This is possible because the type at \extnn{seem} expects the source \ps{\exnn{cat}} of \extnn{sleep} to still be open when the two combine. In other words, we delayed filling the \ps{\exnn{cat}} slot, effectively moving the node \exnn{cat} upwards in the AM tree. Linguistically, the tree in Fig.~\ref{fig:upwardsPercSeem}e makes more sense for this raising construction; better matching conventional notions of syntax.

% We call the process of turning the graph in Fig.~\ref{fig:upwardsPercSeem}d into the one in Fig.~\ref{fig:upwardsPercSeem}e a \emph{percolation}. This is an example of the percolation we call \textbf{P1}, which is schematically shown in Fig.~\ref{fig:percolations}a. In essence, the grandchild of two \app{} operations can be percolated up to become a child of its grandparent by adding its corresponding placeholder source \ps{\nn{n}}, including its request $\tau$ at the parent, to the request of \ps{\nn{p}} at the grandparent's type\todo{This description is a mess. need better notation?}.

% Note that this percolation does not work if either of the edges is a \modify{} edge. If the bottom edge were a \modify{} edge, moving it up the tree would mean that the modifer would modify the wrong node, changing the evaluation result. If the top edge were a \modify{} edge, we cannot update the grandparent's type accordingly, since \modify{} operations, unlike \app{} operations, are not allowed to introduce new sources.



% \paragraph{Unrolled graphs.} We can use this idea of a percolation to obtain AM types that create reentrancies. 

% First, we \emph{unroll} a graph $G$ by \sortof{splitting} all reentrancies like in Fig.~\ref{fig:provisionalAM}d.
% Such an unrolled graph does not represent reentrancies directly, but instead uses \emph{reference nodes} that have special labels, like the node labeled \textsf{REF}-\exnn{cat} here. When merging each reference node with the node it refers to, one obtains the original graph again. We can obtain an AM dep-tree for the unrolled graph with Lemma~\ref{lem:treeAM}.
% %We say an unrolled graph $U$ is \emph{equivalent} to a graph $G$ if resolving all reference nodes in $U$ this way yields $G$. Here, the node-indexed tree in (d) is equivalent to the graph in (b).

% %There are multiple ways of creating a node-indexed tree for a given graph, since all (undirected) cycles in the graph could be split at any node. Further below, we will find that some restrictions apply to the node-indexed tree to obtain only valid AM trees in the and, and we will present a method to obtain all node-indexed trees matching the restrictions there.

% What happens now when we try to percolate the reference node upwards in the AM dep-tree? We can, just as in P1, add the grandchild source \ps{\exnn{cat}} to the request of the parent source \ps{\exnn{sleep}} in the grandparent, yielding the new constant ${\G{want}^P}'$ in Fig.~\ref{fig:provisionalAM}g. However, instead of moving the reference node up, we simply delete it here, yielding the AM dep-tree in Fig.~\ref{fig:provisionalAM}f. We can do this because, in this new AM dep-tree, when $\G{sleep}^P$ combines with ${\G{want}^P}'$, its \ps{\exnn{cat}} merges with the \ps{\exnn{cat}} source ${\G{want}^P}'$ already has, creating the exact reentrancy that the reference node represented. That is, the AM dep-tree after the percolation evaluates to the original graph in Fig.~\ref{fig:provisionalAM}a. We call this percolation \textbf{P2} and show its schema in Fig.~\ref{fig:percolations}b.

% Unlike for P1, there is a variant P3 of P2 where the upper edge is a \modify{} edge (Fig.~\ref{fig:percolations}c). Like P2, P3 removes the reference node, but P3 does not need to change any types: since the parent has the \ps{\nn{n}} source already, the modification will unify the source names appropriately as is.

% % If in this scenario the edge between \tnn{\alpha} and \tnn{\beta} is a \modify{\src{X}} edge instead, then we can do the same percolation to move the \app{\src{Y}} edge up, but only for the case where the \src{Y} source is already contained in the type at \tnn{\alpha} (otherwise, the operation would change the type at \tnn{\alpha}, which is not allowed for \modify{} operations).

% To resolve all reentrancies at a node \nn{n}, we move each node up to its \emph{percolation target}. The percolation target for all AM dep-tree aliases of \nn{n} -- that is the constant creating \nn{n} and all its reference nodes -- is their lowest common ancestor. There, all percolation paths meet and only one AM dep-tree node referring to \nn{n} remains. We first percolate the actual constant up to the percolation target and then percolate all reference nodes upwards until they are consumed by a \textbf{P2} or \textbf{P3} (note that \textbf{P1} can move reference nodes upwards without deleting them). Percolations beyond the percolation target are optional.

% In Appendix~\todo{}, we introduce one more rare type of percolation \textbf{P4} (used for example for raising constructions within relative clauses; \textbf{P4} is not applicable in resolving reentrancies, but can be optionally applied afterwards).
% % and prove the following lemma.
% % \begin{lemma}\label{lem:reentrancies}
% % For every AM dep-tree $t$ with placeholder source names that evaluates to a given graph $G$ there is an AM dep-tree $t'$ with canonical constants that evaluates to an unrolled graph of $G$ such that $t'$ can be transformed into $t$ with a sequence of percolations \textbf{P1-P4}.
% % \end{lemma}

% The general idea to obtain any AM dep-tree for a given graph $G$ then is to unroll $G$ into an unrolled graph $U$, obtain an AM dep-tree with canoncical source names for $U$ with Lemma~\ref{lem:treeAM}, and obtain the final AM dep-tree (with placeholder source names) from there with percolations.

% \todo{fix the rest of this subsection: describe algorithm, use one graph as example (bunch of nodes, mod component in color, schematic not linguistic)}
% We obtain a node-index tree with the desired properties using the following algorithm (the proto-AM-tree then inherits the properties automatically).

% We process all edges of the semantic graph (with edge directions normalized with respect to constant-attachment), starting at the root, adding edges and nodes to the node-indexed tree as we go.

% \todo{this, and particularly the paragraph after, may be hard to understand without pictures. I don't know if we can cut it; if we don't I'll add pictures or reuse the given example}
% In a first pass, we only travel along edges in forward direction. We add all edges and nodes that we encounter to the node-indexed tree $\Gamma$. When we encounter a node a second time, we add a reference node to $\Gamma$ instead and we don't travel through the outgoing edges a second time. All edges added this way correspond to downward edges in the node-index tree and thus \app{} edges in the proto-AM-tree. Therefore, all nodes and reference nodes added this way can be straightforwardly percolated to their percolation target.

% After this procedure is complete, several connected components of not yet processed nodes may remain, that could not be reached by going through edges in forward direction (such as \exnn{little} in Fig.~\ref{fig:provisionalAM}b). Each such component $C$ is connected to the component $M$ of already processed nodes by edges pointing from $C$ to $M$ (if the edge went the other way, it would have been covered in the first, \sortof{forward} pass). We define $D$ to be the set of nodes in $M$ that have an incoming edge from $C$, and define $\nn{x}$ as their lowest common ancestor in $M$. We then pick one edge from $C$ to $\nn{x}$ and split all other edges from $C$ to $M$, introducing reference nodes for the nodes in $M$ where we split\todo{example}. The connecting edge between $C$ and $M$ must connect at $\nn{x}$, because \todo{}. If there is no edge from $C$ to $\nn{x}$, there is no AM tree evaluating to the semantic graph using the edge-constant groupings made above, and the decomposition fails. If there are multiple such edges, each is a valid choice and we obtain structurally different AM trees depending on which one we pick. %In practice, we find that this occurs very rarely and we simply select an arbitrary edge.

% We then iterate this process for the component $C$, using the node connected to $\nn{x}$ as the new root; we continue this process until all nodes and edges are covered. We present a technical description of this procedure, and a proof that it yields exactly all node-indexed trees with the desired properties, in Appendix~\todo{}

% \subsection{Unrolling the graph}

% At first glance, the above procedure may look like many different AM dep-trees can be obtained with it -- after all, there are many ways to unroll a graph. However, we can show that most ways of unrolling $G$ either lead to the same final AM dep-tree or do not lead to a well-typed AM dep-tree at all; in effect, the final AM dep-tree is still quite restricted even if we allow type annotations.

% A \modify{} edge cannot be percolated upwards. An \app{} edge with child \nn{n} cannot be percolated past a \modify{} edge, except if the parent has a 

% \paragraph{Forward paths.} To see this, we define some properties that the unrolled graph $U$ must satisfy such that we can resolve all reentrancies with percolations. The first \textbf{Property 1} is that, if an edge $e$ can be traversed in $G$ by only traversing edges (including $e$) in forward direction, then $e$ must point away from the root in $U$. If this property does not hold, then not all nodes can be percolated to their percolation target. To see this, consider the graph in Fig.~\ref{}.\todo{spell out this example}

% Let us assume now that in our graph $G$, there are only such edges (that can be traversed from the root by only traversing edges in forward direction). Then we must unroll $G$ in a way that traverses all edges in forward direction, otherwise Property 1 is violated. This leaves us little choice in the unrolling procedure -- the only choice is which of the aliases for a node has the original constant, and which are reference nodes. However, in the percolation step all aliases get percolated to the same target. Thus, whichever alias in $U$ carries the constant, after percolation to resolve the reentrancies, the AM dep-tree is the same. Therefore, under this assumption, the only choices to make when obtaining an AM dep-tree with placeholder sources is the partitioning into blobs, and optional percolations beyond resolving reentrancies.

% \paragraph{Modifier components.} Let us now consider the general case, where there are also edges that cannot be traversed by forward paths\todo{define above}. In this case too, specific restrictions apply. We define the \emph{forward component} $F$ of $G$ as the set of all nodes that can be reached by forward paths from the root; $F$ must be unrolled as described above. Removing $F$ from $G$ leaves us with possibly multiple connected components $C_1,\dots,C_n$. Each component $C_i$ is connected to $F$ with edges pointing from $C_i$ to $F$ (otherwise some nodes of $C_i$ could be reached by forward paths). We write $D_i$ for the set of nodes in $F$ with an incoming edge from $C_i$. \textbf{Property 2} then is: in $U$, for each $C_i$, exactly one edge $e_i$ between original nodes of $C_i$ and $D_i$ remains, which is an edge between some node $r_i$ in $C_i$ and the lowest common ancestor of $D_i$,  $\text{LCA}\of{D_i}$ (lowest common ancestor with respect to constant-normalized edge directions in $G$). This gives a scenario like the one shown in Fig.~\todo{}: the connected component attached to $U$ at $\text{LCA}\of{D_i}$ is connected via $r_i$ and contains exactly $C_i$ and possible reference nodes to $D_i$.

% The reason behind this Property 2 goes back to the principle that percolating a node \nn{n} past a \modify{} edge is only possible if the prospective new parent already has an \ps{\nn{n}} source (see above). First note that every edge between $C_i$ and $D_i$ will become a \modify{} edge by Lemma~\ref{lem:treeAM}. If Property 2 holds, evert source we need to percolate past the \modify{} edge stemming from the edge $e_i$ between $r_i$ and $\text{LCA}\of{D_i}$ is a placeholder source \ps{\nn{d}} for a node $\nn{d}\in D_i$. We can percolate it past that \modify{} edge because we can get \ps{\nn{d}} into the type of $\text{LCA}\of{D_i}$ with percolations \textbf{P1}.\todo{example}

% If however a \sortof{connection node} other than $\text{LCA}\of{D_i}$ is chosen, or multiple edges between $C_i$ and $D_i$ are kept (unrolling the graph instead by splitting $C_i$ apart), not all resulting reference nodes can reach their percolation targets with \textbf{P1-3}; illegal percolations past \modify{} edges would be necessary. We prove this in the form the the following Lemma in Appendix~\todo{}.\todo{example}.

% \begin{lemma}\label{lem:unrollingProperties}
% If $U$ does not have Properties 1-2, its reentrancies cannot be resolved with percolations \textbf{P1-3}.
% \end{lemma}

% % All other nodes between $C_i$ and $D_i$ go from an original node in $C_i$ to a reference node of a node in $D_i$. \todo{example} \todo{see this as $C_i$ being a subtree of $r_i$ in $U$; recursiveness}

% The idea of unrolling along forward paths and splitting off modifier components continues recursively within each modifier component $C_i$ (including the reference nodes to $D_i$, with $r_i$ taking the place of the root. Properties~1 and~2 must hold in this recursive fashion.\todo{say this before the lemma?}

% % ; that is we can see the whole component of $C_i$ to modify $F$. To unroll the graph however, we must \sortof{cut} all these connections except one. We write $D_i$ for the set of nodes in $F$ with an incoming edge from $C_i$.  In the unrolled graph then, one of the nodes in $C_i$, let us call it $r_i$, is a direct child of one of the nodes in $D_i$ and the rest of $C_i$ (as well as reference nodes to the other nodes in $D_i$) is a descendent of $r_i$.

% % \todo{notion of descendant etc in $U$}

% % Property 2: In $U$, one node $\tnn{r}_i$ of $C_i$ is a direct child of the lowest common ancestor of $D_i$ and all nodes of $C_i$ are below it. \todo{refnodes to $D_i$}


% Which edge $e_i$ to keep, i.e.~which node in $C_i$ to chose as the \sortof{local root} $r_i$, is a meaningful choice (if there are multiple such edges), yielding structurally different AM trees. If there is no such edge $e_i$, one cannot obtain an AM dep-tree evaluating to $G$ with this blob partition (this follows directly from Lemma~\ref{lem:unrollingProperties}).

==> rules-projective.tex <==
\begin{figure}
  \centering 
\definecolor{LGray}{gray}{0.9}

    \small
\begin{tabular}{@{}c@{}}
\rowcolor{LGray}
  \infer{Init}{
    s = \graphCost{i}{G}
    \quad
    G \neq \bot
  }{
    \pitem{i}{i+1}{i}{\tp{G}}{s}
  }\\
  \infer{Skip-R}{\hspace{-3pt}\pitem{i}{k}{r}{\tau}{s}
    \quad
    s' = \graphCost{k}{\bot}+\edgeCost{0}{k}{\lignore}
  }{
    \pitem{i}{k+1}{r}{\tau}{s+s'}
  }\hspace{-5pt}\\
\rowcolor{LGray}
%   \infer{Skip-L}{
%     \pitem{i}{k}{r}{\tau}{s}
%     \quad
%     s' = \score(\bot,i-1)+\score\of{0\xrightarrow{\text{\tiny \lignore}}i-1}
%   }{
%     \pitem{i-1}{k}{r}{\tau}{s+s'}
%   }
  \begin{minipage}{0.9\linewidth}
  \begin{prooftree}
  \AxiomC{\stackanchor{$\pitem{i}{k}{r}{\tau}{s}$}
                {$s' = \graphCost{i-1}{\bot}+\edgeCost{0}{i-1}{\lignore}$}
        }
  \RightLabel{Skip-L}
  \UnaryInfC{$\pitem{i-1}{k}{r}{\tau}{s+s'}$}
  \end{prooftree}
  \end{minipage}\\
  \begin{minipage}{0.9\linewidth}
  \begin{prooftree}
  \AxiomC{\stackanchor{$\pitem{i}{j}{r_1}{\tau_1}{s_1} \quad \pitem{j}{k}{r_2}{\tau_2}{s_2}$}
                {$\tau = \oper(\tau_1, \tau_2) \;\mbox{defined} \quad s = \edgeCost{r_1}{r_2}{\oper}$}
        }
  
  \RightLabel{Arc-R [\oper]}
  \UnaryInfC{$\pitem{i}{k}{r_1}{\tau}{s_1+s_2+s}$}
  \end{prooftree}
  \end{minipage}\\
  %~ \infer{Arc-R [o]}{
    %~ \pitem{i}{j}{r_1}{\tau_1}{s_1}
    %~ \quad
    %~ \pitem{j}{k}{r_2}{\tau_2}{s_2}
    %~ \\
    %~ \tau = o(\tau_1, \tau_2) \;\mbox{defined}
    %~ \quad
    %~ s = \score(o[r_1, r_2])
  %~ }{
    %~ \pitem{i}{k}{r_1}{\tau}{s_1+s_2+s}
  %~ }\strut\\\strut
\rowcolor{LGray}
  \begin{minipage}{0.9\linewidth}
      \begin{prooftree}
      \AxiomC{\stackanchor{$\pitem{i}{j}{r_1}{\tau_1}{s_1} \quad \pitem{j}{k}{r_2}{\tau_2}{s_2}$}
                    {$\tau = \oper(\tau_2, \tau_1) \;\mbox{defined} \quad s = \edgeCost{r_2}{r_1}{\oper}$}
            }
      
      \RightLabel{Arc-L [\oper]}
      \UnaryInfC{$\pitem{i}{k}{r_2}{\tau}{s_1+s_2+s}$}
      \end{prooftree}
    \end{minipage}\\
    \infer{Root}{
    \pitem{1}{n+1}{r}{\emptytype}
    \quad
    s' = \edgeCost{0}{r}{\lroot}
  }{
    \pitem{0}{n+1}{r}{\emptytype}{s+s'}
  }

  %~ \infer{\todo{Arc-L [o]}}{
    %~ \pitem{i}{j}{r_1}{\tau_1}{s_1}
    %~ \quad
    %~ \pitem{j}{k}{r_2}{\tau_2}{s_2}
    %~ \\
    %~ \tau = o(\tau_2, \tau_1) \;\mbox{defined}
    %~ \quad
    %~ s = \score(o[r_2, r_1])
  %~ }{
    %~ \pitem{i}{k}{r_2}{\tau}{s_1+s_2+s}
  %~ }
  
  \end{tabular}
  \caption{Rules for the projective and A* decoder.}
  \label{fig:rules-projective}
\end{figure}






%%% Local Variables:
%%% mode: latex
%%% TeX-master: "am-parsing-20"
%%% End:

